A Kernel-Based Approach to Non-Stationary Reinforcement Learning in Metric Spaces

In this work, we propose KeRNS: an algorithm for episodic reinforcement learning in non-stationary Markov Decision Processes (MDPs) whose state-action set is endowed with a metric. Using a non-parametric model of the MDP built with time-dependent kernels, we prove a regret bound that scales with the covering dimension of the state-action space and the total variation of the MDP with time, which quantifies its level of non-stationarity. Our method generalizes previous approaches based on sliding windows and exponential discounting used to handle changing environments. We further propose a practical implementation of KeRNS, we analyze its regret and validate it experimentally.

==> source_arxiv_march_2022/app_efficient_version.tex <==
%\section{\kerns on Representative States - Full Model Updates}
%\label{app:efficient_implementation}
%

%In each episode $k$, \RSkerns keeps and updates sets of representative states $\ReprStates$, actions $\ReprActions$ and next-states $\ReprNextStates$, with cardinalities $\NreprStates, \NreprActions$ and $\NreprNextStates$, respectively. For simplicity, we omit the dependence on $k$ of these sets and their cardinalities. We define the following projections:
%\begin{align*}
%\maptoReprSA(x, a) \eqdef \argmin_{(\bx,\ba) \in \ReprStates\times\ReprActions} \dist{(x,a),  (\bx,\ba)}
%,\quad 
%\maptoReprS(y) \eqdef \argmin_{\by \in \ReprNextStates} \Sdist{y, \by}.
%\end{align*}
%where we also assume to have access to the metric $\Sdistfunc$.
%
%\subsection{Algorithm}
%
%\begin{fdefinition}[kernel weights on representative states]
%	\label{definition:RS-kernel-weights}
%	For any $(x, a) \in \stateactionspace$, we define the weights and the normalized weights on the representative states at step $h$ of episode $k$ as
%	\begin{align*}
%	& \weight_{h,\mapzeta}^{k, s}(x, a) \eqdef \fullkernel\pa{k-s-1, \maptoReprSA(x, a), \maptoReprSA(x_h^s, a_h^s)} 
%	,\quad \normweight_{h, \mapzeta}^{k, s}(x, a) \eqdef \frac{\weight_{h,\mapzeta}^{k, s}(x, a) }{\gencount_{h,\mapzeta}^{k}(x, a)}
%	\end{align*}
%	where $\gencount_{h,\mapzeta}^{k}(x, a) \eqdef \kbeta + \sum_{s=1}^{k-1} \weight_{h,\mapzeta}^{k, s}(x, a)$ are the generalized counts, and $\kbeta > 0$ is a regularization parameter.
%\end{fdefinition}
%
%
%\begin{fdefinition}[empirical MDP on representative states]
%	\label{definition:RS-reward-and-transition-estimator}
%	At time $(s, h) \in [K]\times[H]$, let $(x_h^s, a_h^s, x_{h+1}^s, \obsreward_h^s)$  represent the state, the action, the next state and the reward observed by the algorithm. Before each episode $k$, \RSkerns estimates the rewards and transitions using the data observed up to episode $k-1$: 
%	\begin{align*}
%	\estR_{h,\mapzeta}^k(x, a) \eqdef \sum_{s=1}^{k-1} \normweight_{h,\mapzeta}^{k, s}(x, a) \obsreward_h^s
%	, \quad 
%	\estP_{h,\mapzeta}^k (y|x, a) =  \sum_{s=1}^{k-1} \normweight_{h,\mapzeta}^{k, s}(x, a) \dirac{\maptoReprS(x_{h+1}^s)}(y)
%	\end{align*}
%	where $\dirac{x}$ is the Dirac measure at $x$. Let $\estMDP_k^{\mapzeta}$ be the MDP whose rewards and transitions at step $h$ are $\estR_{h,\mapzeta}^k(x, a)$ and $\estP_{h,\mapzeta}^k (y|x, a)$.
%\end{fdefinition}
%
%% ----------------------------------------------------------------------------
%% RS-KeRNS
%% ----------------------------------------------------------------------------
%\begin{fdefinition}[\RSkerns with full model updates]
%
%In each episode $k$, \RSkerns with \emph{full model updates} proceeds as follows:
%
%\begin{enumerate}
%	\item Build $\estR_{h,\mapzeta}^k$ and $\estP_{h,\mapzeta}^k$ as in Definition \ref{definition:RS-reward-and-transition-estimator}.
%	\item For each $h\in[H]$, with $\algV_{H+1,\mapzeta}^k = 0$,
%	
%	\begin{itemize}
%		\item Compute, for all $(x, a) \in \ReprStates\times\ReprActions $
%		\begin{align*}
%		\tQ_{h,\mapzeta}^k(x, a) = \estR_{h,\mapzeta}^k(x, a) + \estP_{h,\mapzeta}^k \algV_{h+1,\mapzeta}^k(x, a) + \bonus_{h,\mapzeta}^k(x, a):\\
%		\end{align*}
%		\item Define, for any $(x, a)$,
%		\begin{align*}
%		& \algQ_{h,\mapzeta}^k(x, a) = \min_{(\bx,\ba)\in\ReprStates\times\ReprActions} \sqrbrackets{ \tQ_{h,\mapzeta}^k(\bx,\ba) + \lipQ \dist{(x, a), (\bx,\ba)}  } \\
%		& \algV_{h,\mapzeta}^k (x) = \min\pa{H-h+1, \max_{a'}\algQ_{h,\mapzeta}^k(x, a')}
%		\end{align*}			
%	\end{itemize} 
%	
%	\item For $h\in[H]$, choose the action $ a_h^k \in \argmax_a \algQ_{h,\mapzeta}^k(x_h^k, a)$.
%\end{enumerate}
%
%\end{fdefinition}
%\begin{algorithm}[H]
%	\centering
%	\caption{\RSkerns with full model updates}\label{alg:RS-kerns}
%	\begin{algorithmic}[1]
%		\State {\bfseries Input:} global parameters $K$, $H$, $\lipQ$, $\lipR$ , $\lipP$, $\kbeta$, $\cdelta$, $\totalcovdim$, $\ksigma$, $\keta$, $\kW$, $\Smaxdist$, $\maxdist$.
%		\State Initialize transition history: $\cT_h = \emptyset$ for all $h\in[H]$.
%		\State Initialize representative states, actions and next states: $\ReprStates = \emptyset$, $\ReprActions = \emptyset$, $\ReprNextStates=\emptyset$.
%		\For{episode $k=1, \ldots, K$}
%		\State get initial state $x_1^k$
%		\State compute $(\algQ_{h,\mapzeta}^k)_h$ using data $(\cT_h)_h$ and kernel backward induction (Alg. \ref{alg:RS-kernel_backward_induction}).
%		\For{$h = 1, \ldots, H$}
%		\State execute $a_h^k = \argmax_a \algQ_{h, \mapzeta}^k(x_h^k, a)$, observe reward $\obsreward_h^k$ and next state $x_{h+1}^k$
%		\State update $\ReprStates$, $\ReprActions$ and $\ReprNextStates$ using $\braces{ (x_h^k, a_h^k), x_{h+1}^k}$ (Alg. \ref{alg:update-representative-states-main-text})
%		\State update model using $\braces{\maptoReprSA(x_h^k, a_h^k), \maptoReprS(x_{h+1}^k), \obsreward_h^k}$ (see Alg. \ref{alg:online-kerns-updates} for online updates)
%		\EndFor
%		\EndFor 
%	\end{algorithmic}
%\end{algorithm} 

%\begin{algorithm}[H]
%	\centering
%	\caption{Update Representative States and Actions}\label{alg:update-representative-states}
%	\footnotesize
%	\begin{algorithmic}[1]
%		\State {\bfseries Input: $\ReprStates$, $\ReprActions$, $\braces{x_h^k, a_h^k, x_{h+1}^k}$}.
%		\If{$\min_{(\bx,\ba)\in\ReprStates\times\ReprActions}\dist{(\bx,\ba), (x_h^k, a_h^k)} > \maxdist$}
%			\State $\ReprStates = \ReprStates \cup \braces{x_h^k}$, \ \  $\ReprActions = \ReprActions \cup \braces{a_h^k}$
%		\EndIf 
%		\If{$\min_{\by\in\ReprNextStates}\Sdist{\bx, x_{h+1}^k} > \Smaxdist$}
%			\State $\ReprNextStates = \ReprNextStates \cup \braces{x_{h+1}^k}$
%		\EndIf 
%			\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}[H]
%	\centering
%	\caption{Kernel Backward Induction on Representative States}\label{alg:RS-kernel_backward_induction}
%	\begin{algorithmic}[1]
%		\State {\bfseries Input:} $k$, $H$, $\fullkernel$, $\lipQ$, $\kbeta$ , $\estR_{h,\mapzeta}^k(\bx, \ba)$, $\estP_{h,\mapzeta}^k(\by|\bx, \ba)$ for all $h \in [H], (\bx,\ba,\by)\in\ReprStates\times\ReprActions\times\ReprNextStates$. 
%		\State {\bfseries Initialization: } $\algV_{H+1, \mapzeta}(x) = 0$ for all $x\in\statespace$
%		\For{$h = H,\ldots, 1$}
%		\For{$(\bx, \ba) \in \ReprStates\times\ReprActions$}
%			\State $\tQ_{h,\mapzeta}(\bx, \ba) = \estR_{h,\mapzeta}^k(\bx, \ba) + \estP_{h,\mapzeta}^k \algV_{h+1, \mapzeta}(\bx, \ba) + \bonus_{h,\mapzeta}^k(\bx, \ba)  $ 
%		\EndFor
%		\State{\color{darkgreen2} // Interpolated $Q$-function. Defined, but not computed for all $(x, a)$}
%		\State $Q_{h, \mapzeta}(x, a) = \underset{(\bx,\ba) \in\ReprStates\times\ReprActions }{\min}\pa{\tQ_{h, \mapzeta}(\bx,\ba)+\lipQ \dist{(x,a), (\bx,\ba)}}$ 
%		\For{$\by \in \ReprNextStates$}
%		\State $\algV_{h, \mapzeta}(\by) = \min\pa{H-h+1, \max_{a}\algQ_{h,\mapzeta}(\by, a)}$ 
%		\EndFor
%		\EndFor 
%		\State {\bfseries Return:} $(\algQ_{h,\mapzeta})_{h\in[H]}$
%	\end{algorithmic}
%\end{algorithm} 

%\subsection{Regret Bounds}


%\begin{fcorollary}
%	\label{corollary:lipschitznes_of_kerns_with_gaussian_kernel}
%	Let $\timekernel:\NN \to [0, 1]$, consider the following kernel
%	\begin{align*}
%	\fullkernel(t, u, v) = \timekernel(t) \exp\pa{-\dist{u, v}^2/(2\ksigma^2)}
%	\end{align*}
%	where $u, v\in\stateactionspace$. Recall the definition of the weights 
%	\begin{align*}
%	\weight_h^{k, s}(x, a) = \fullkernel(k-s-1, (x, a), (x_h^s,a_h^s)), \; \weight_{h,\mapzeta}^{k, s}(x, a) \eqdef \fullkernel\pa{k-s-1, \maptoReprSA(x, a), \maptoReprSA(x_h^s, a_h^s)} 
%	\end{align*}
%	and consider the functions
%	\begin{align*}
%	& g_1(x, a) = \frac{\sum_{s=1}^{k-1} \weight_h^{k, s}(x, a) Y_s}{\kbeta+\sum_{s=1}^{k-1} \weight_h^{k, s}(x, a)}
%	,\quad
%	g_1^{\mapzeta}(x, a) = \frac{\sum_{s=1}^{k-1} \weight_{h,\mapzeta}^{k, s}(x, a) Y_s}{\kbeta+\sum_{s=1}^{k-1} \weight_{h,\mapzeta}^{k, s}(x, a)}
%	, \\ 
%	& g_2(x, a) = \sqrt{\frac{1}{\kbeta+\sum_{s=1}^{k-1} \weight_h^{k, s}(x, a)}}
%	, \quad
%	g_2^{\mapzeta}(x, a) = \sqrt{\frac{1}{\kbeta+\sum_{s=1}^{k-1} \weight_{h,\mapzeta}^{k, s}(x, a)}}
%	,\\
%	& g_3(x, a) = \frac{1}{\kbeta+\sum_{s=1}^{k-1} \weight_h^{k, s}(x, a)}
%	,\quad
%	g_3^{\mapzeta}(x, a) = \frac{1}{\kbeta+\sum_{s=1}^{k-1} \weight_{h,\mapzeta}^{k, s}(x, a)}
%	.
%	\end{align*}
%	where $(Y_s)_{s=1}^{k-1}$ is an arbitrary sequence. 
%	Then, $g_1$, $g_2$ and $g_3$ are \lipschitz continuous, whose \lipschitz constants are bounded by $L_1$, $L_2$ and $L_3$, respectively, with
%	\begin{align*}
%	L_1 = \frac{ 4 \max_s\abs{Y_s}}{\ksigma} & \pa{1+\sqrt{\logplus(k/\kbeta)}}
%	,\quad 
%	L_2 = \frac{1+\sqrt{\logplus(k/\kbeta)}}{2 \kbeta^{1/2}\ksigma}
%	,\quad 
%	L_3 = \frac{1+\sqrt{\logplus(k/\kbeta)}}{\kbeta \ksigma}
%	\end{align*}
%	Furthermore, we have, for any $(x, a)$ and for $i \in \braces{1, 2, 3}$,
%	\begin{align*}
%		\abs{g_i^{\mapzeta}(x, a)-g_i(\maptoReprSA(x, a))} \leq L_i \max_s \dist{(x_h^s, a_h^s), \maptoReprSA(x_h^s, a_h^s)}.
%	\end{align*}
%\end{fcorollary}
%\begin{proof} First, let's prove that $g_1$, $g_2$ and $g_3$ are Lipschitz continuous.
%	From Lemma \ref{lemma:gaussian-case-weighted-average-and-bonuses-are-lipschitz}, taking $z= (\dist{(x,a),(x_h^s,a_h^s)})_{s=1}^{k-1}$ and $y = (\dist{(x',a'),(x_h^s,a_h^s)})_{s=1}^{k-1}$ we have
%	\begin{align*}
%	\abs{g_1(x, a)-g_1(x', a')} \leq \frac{ 4 \max_s\abs{Y_s}}{\ksigma} \pa{1+\sqrt{\logplus(k/\kbeta)}} \max_{s\in[k-1]} \abs{z_s - y_s}.
%	\end{align*}
%	By the triangle inequality, we have, for all $s$,
%	\begin{align*}
%	\abs{z_s - y_s} = \abs{ \dist{(x,a),(x_h^s,a_h^s)} - \dist{(x',a'),(x_h^s,a_h^s)}} \leq \dist{(x,a),(x',a')}
%	\end{align*}
%	which implies
%	\begin{align*}
%	\abs{g_1(x, a)-g_1(x', a')} \leq \frac{ 4 \max_s\abs{Y_s}}{\ksigma} \pa{1+\sqrt{\logplus(k/\kbeta)}} \dist{(x,a),(x',a')}.
%	\end{align*}
%	giving the \lipschitz constant of $g_1$. The \lipschitz constants of $g_2$ and $g_3$ follow similarly from Lemma \ref{lemma:gaussian-case-weighted-average-and-bonuses-are-lipschitz}.
%	
%	Now, let's bound the differences $\abs{g_i^{\mapzeta}(x, a)-g_i(\maptoReprSA(x, a))}$. Let $\chi(s) = \timekernel(k-s-1)$. For $i=1$,  and applying again Lemma  \ref{lemma:gaussian-case-weighted-average-and-bonuses-are-lipschitz}, we have
%	\begin{align*}
%		& \abs{g_1^{\mapzeta}(x, a)-g_1(\maptoReprSA(x, a))}  \\
%		& = \abs{
%				\frac{\sum_{s=1}^{k-1} \chi(s) \exp\pa{-\frac{\dist{\maptoReprSA(x,a), \maptoReprSA(x_h^s,a_h^s)}^2}{2\ksigma^2}} Y_s}{\kbeta+\sum_{s=1}^{k-1} \chi(s) \exp\pa{-\frac{\dist{\maptoReprSA(x,a), \maptoReprSA(x_h^s,a_h^s)}^2}{2\ksigma^2}}}
%				-
%				\frac{\sum_{s=1}^{k-1} \chi(s) \exp\pa{-\frac{\dist{\maptoReprSA(x,a), (x_h^s,a_h^s)}^2}{2\ksigma^2}} Y_s}{\kbeta+\sum_{s=1}^{k-1} \chi(s) \exp\pa{-\frac{\dist{\maptoReprSA(x,a), (x_h^s,a_h^s)}^2}{2\ksigma^2}}}
%		       } \\
%	    & \leq \frac{ 4 \max_s\abs{Y_s}}{\ksigma} \pa{1+\sqrt{\logplus(k/\kbeta)}} \max_{s\in[k-1]} \abs{\dist{\maptoReprSA(x,a), \maptoReprSA(x_h^s,a_h^s)} - \dist{\maptoReprSA(x,a), (x_h^s,a_h^s)}} \\
%	    & \leq \frac{ 4 \max_s\abs{Y_s}}{\ksigma} \pa{1+\sqrt{\logplus(k/\kbeta)}} \max_{s\in[k-1]} \dist{\maptoReprSA(x_h^s,a_h^s), (x_h^s,a_h^s)},
%	\end{align*}
%	where in the last line we used the triangle inequality.  The proof for $i \in \braces{2, 3}$ also follow from Lemma \ref{lemma:gaussian-case-weighted-average-and-bonuses-are-lipschitz}.
%\end{proof}



%% ---------------------------
%% Error in P
%% ---------------------------
%\begin{flemma}
%	\label{lemma:error-in-P-when-usin-representative-states}
%	Let $V$ be an arbitrary $\lipQ$-\lipschitz function bounded by $H$. Then, for any $(x, a)$,
%	\begin{align*}
%		\abs{\pa{\estP_h^k - \estP_{h,\mapzeta}^k}V(x, a)} 
%		\leq & \lipQ \max_{s\in[k-1]}\Sdist{x_{h+1}^s, \maptoReprS(x_{h+1}^s)} \\
%		& + \frac{4H}{\ksigma}\pa{1+\sqrt{\logplus(k/\kbeta)}}\pa{ \dist{(x,a),\maptoReprSA(x,a)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)} }
%	\end{align*}
%\end{flemma}
%\begin{proof}
%	We have
%	\begin{align*}
%		\abs{\pa{\estP_h^k - \estP_{h,\mapzeta}^k}V(x, a)} \leq 
%		&\abs{ \sum_{s=1}^{k-1} \normweight_h^{k,s}(x,a)V(x_{h+1}^s) -  \sum_{s=1}^{k-1} \normweight_h^{k,s}(x,a)V(\maptoReprS(x_{h+1}^s)) } \\
%		&  + \abs{ \sum_{s=1}^{k-1} \normweight_h^{k,s}(x,a)V(\maptoReprS(x_{h+1}^s)) -  \sum_{s=1}^{k-1} \normweight_h^{k,s}(\maptoReprSA(x,a))V(\maptoReprS(x_{h+1}^s)) } \\
%		& + \abs{ \sum_{s=1}^{k-1} \normweight_h^{k,s}(\maptoReprSA(x,a))V(\maptoReprS(x_{h+1}^s)) -  \sum_{s=1}^{k-1} \normweight_{h,\mapzeta}^{k,s}(x,a)V(\maptoReprS(x_{h+1}^s)) } 
%	\end{align*}
%	and the result follows immediately from Corollary \ref{corollary:lipschitznes_of_kerns_with_gaussian_kernel}.
%\end{proof}


%% ---------------------------
%% Error in R
%% ---------------------------
%\begin{flemma}
%	For any $(x, a)$, we have
%	\label{lemma:error-in-R-when-usin-representative-states}
%	\begin{align*}
%	\abs{\estR_h^k(x, a) - \estR_{h,\mapzeta}^k(x, a)} 
%	\leq  \frac{4}{\ksigma}\pa{1+\sqrt{\logplus(k/\kbeta)}}\pa{ \dist{(x,a),\maptoReprSA(x,a)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)} }
%	\end{align*}
%\end{flemma}
%\begin{proof}
%	It follows from a similar decomposition as in the proof of Lemma \ref{lemma:error-in-P-when-usin-representative-states} and an application of Corollary \ref{corollary:lipschitznes_of_kerns_with_gaussian_kernel}.
%\end{proof}

%% ---------------------------
%% Error in bonus
%% ---------------------------
%\begin{flemma}
%	\label{lemma:error-in-bonus-when-usin-representative-states}
%	For any $(x, a)$, we have,
%	\begin{align*}
%		\abs{ \bonus_h^k(x, a) - \bonus_{h,\mapzeta}^k(x, a)} \lesssim  
%		\frac{H}{\ksigma}\pa{1+\frac{1}{2 \kbeta^{1/2}}}\pa{ \dist{(x,a),\maptoReprSA(x,a)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)}}
%	\end{align*}
%\end{flemma}
%\begin{proof}
%	From the definition of the bonuses (Def. \ref{def:exploration-bonuses}) and Corollary \ref{corollary:lipschitznes_of_kerns_with_gaussian_kernel}, we have
%	\begin{align*}
%		& \abs{ \bonus_h^k(x, a) - \bonus_{h,\mapzeta}^k(x, a)}  \\
%		& \lesssim
%		 H \abs{ \sqrt{  \frac{1}{\gencount_h^k(x, a)}} - \sqrt{\frac{1}{\gencount_{h,\mapzeta}^k(x, a)}}} 
%		  + \kbeta H\abs{ \frac{1}{\gencount_h^k(x, a)} - \frac{1}{\gencount_{h,\mapzeta}^k(x, a)}  } \\
%		 & \leq  H \abs{ \sqrt{  \frac{1}{\gencount_h^k(x, a)}} - \sqrt{\frac{1}{\gencount_{h}^k(\maptoReprSA(x, a))}}} 
%		        + H \abs{ \sqrt{  \frac{1}{\gencount_h^k(\maptoReprSA(x, a))}} - \sqrt{\frac{1}{\gencount_{h,\mapzeta}^k(x, a)}}}  \\
%		 & +  \kbeta H\abs{ \frac{1}{\gencount_h^k(x, a)} - \frac{1}{\gencount_{h}^k(\maptoReprSA(x, a))}  }
%		 + \kbeta H\abs{ \frac{1}{\gencount_h^k(\maptoReprSA(x, a))} - \frac{1}{\gencount_{h,\mapzeta}^k(x, a)}  } \\
%		 %
%		 & \leq \frac{H(1+\sqrt{\logplus(k/\kbeta))}}{2 \kbeta^{1/2}\ksigma}\pa{ \dist{(x,a),\maptoReprSA(x,a)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)}} \\
%		 & + \frac{H(1+\sqrt{\logplus(k/\kbeta)})}{\ksigma}\pa{ \dist{(x,a),\maptoReprSA(x,a)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)}}
%	\end{align*}
%\end{proof}

%% -----------------------------------------------------------------
%% Important technical Lemma
%% -----------------------------------------------------------------
%\begin{flemma}
%	\label{lemma:technical-inequality-for-KeRNS-with-minimum}
%	We have
%	\begin{align*}
%		\algQ_{h, \mapzeta}^k(x, a) & \eqdef \underset{(\bx,\ba) \in\ReprStates\times\ReprActions }{\min}\pa{\tQ_{h, \mapzeta}^k(\bx,\ba)+\lipQ \dist{(x,a), (\bx,\ba)}} \\
%		& = \underset{s\in[k-1], h\in[H]}{\min}\pa{\tQ_{h, \mapzeta}^k(x_h^s, a_h^s)+\lipQ \dist{(x,a), \maptoReprSA(x_h^s, a_h^s)}} 
%	\end{align*}
%\end{flemma}
%\begin{proof}
%	By construction, we have 
%	\begin{align*}
%		\braces{\maptoReprSA(x_h^s,a_h^s): s\in[k-1], h \in [H]} = \ReprStates\times\ReprActions.
%	\end{align*}
%	since, $\forall (s,h)$, we have $\maptoReprSA(x_h^s,a_h^s) \in \ReprStates\times\ReprActions$ and, for any $(\bx, \ba) \in \ReprStates\times\ReprActions$, there exists $(s,h)$ such that $(\bx, \ba) = (x_h^s,a_h^s)$ by construction.
%	
%	
%	Together with the fact that $\tQ_{h, \mapzeta}^k(x_h^s, a_h^s) = \tQ_{h, \mapzeta}^k(\maptoReprSA(x_h^s, a_h^s))$, this concludes the proof.
%\end{proof}

%% -----------------------------------------------------------------
%% Important Lemma: bouding error in Q_h^k when using representative states
%% -----------------------------------------------------------------
%\begin{flemma}
%	\label{lemma:diff-between-Q-in-kerns-and-RS-kerns}
%	The difference between the $Q$-values computed by \kerns and \RSkerns are bounded as follows
%	\begin{align*}
%		\sup_{x, a}\abs{ \algQ_h^k(x, a) - \algQ_{h,\mapzeta}^k(x, a)} \lesssim \pa{\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H}(H-h+1).
%	\end{align*}
%\end{flemma}
%\begin{proof}
%	We proceed by induction on $h$. Let
%	\begin{align*}
%		\epsilon_h \eqdef \pa{\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H}(H-h+1).
%	\end{align*}
%	For $h=H+1$, $\epsilon_h = 0$ and the claim holds. 
%	
%	Now, assume that the claim is true for $h+1$. In this case, we have, for any $x$, 
%	\begin{align*}
%		& 
%		\abs{\algV_{h+1}^{k}(x) - \algV_{h+1,\mapzeta}^{k}(x)}
%		\\
%		& 
%		= \abs{\min \pa{H-h, \max_a\algQ_{h+1}^{k}(x, a)} - \min \pa{H-h, \max_a\algQ_{h+1,\mapzeta}^{k}(x, a)}}
%		\\
%		& 
%		\leq
%		\abs{\max_a\algQ_{h+1}^{k}(x, a) - \max_a\algQ_{h+1,\mapzeta}^{k}(x, a)}
%		 \\
%		 & 
%		 \leq \max_{a}\abs{\algQ_{h+1}^{k}(x, a) - \algQ_{h+1,\mapzeta}^{k}(x, a)} \leq \epsilon_{h+1},
%	\end{align*}
%	where we used induction hypothesis and the fact that, for any $a, b, c \in \RR$, we have $\abs{\min(a, b) -\min(a, c)} \leq \abs{b-c}$ (Fact~\ref{fact:small-useful-result-with-min}).
%	
%	For any $(x_h^s, a_h^s)$ with $s\in[k-1]$, we have
%	\begin{align*}
%		& \abs{\tQ_{h}^k(x_h^s, a_h^s) -\tQ_{h, \mapzeta}^k(x_h^s, a_h^s)} \\
%		& \leq  \abs{\estR_h^k(x_h^s, a_h^s) - \estR_{h,\mapzeta}^k(x_h^s, a_h^s)}
%		     +  \abs{\bonus_h^k(x_h^s, a_h^s) - \bonus_{h,\mapzeta}^k(x_h^s, a_h^s)} \\
%		   &\quad + \abs{\pa{\estP_h^k - \estP_{h,\mapzeta}^k}\algV_{h+1}^{k}(x_h^s, a_h^s) 
%		   + \estP_{h,\mapzeta}^k\pa{ \algV_{h+1}^{k} - \algV_{h+1,\mapzeta}^{k}}(x_h^s, a_h^s)} \\
%	   & \lesssim \epsilon_{h+1} +  \lipQ \max_{s'\in[k-1]}\Sdist{x_{h+1}^{s'}, \maptoReprS(x_{h+1}^{s'})} \\
%	   & +  \frac{H}{\ksigma}\pa{ \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)} + \max_{s'\in[k-1]} \dist{(x_h^{s'},a_h^{s'}),\maptoReprSA(x_h^{s'},a_h^{s'})} }
%	\end{align*}
%	where, in the last line, we used the induction hypothesis and lemmas \ref{lemma:error-in-P-when-usin-representative-states}, \ref{lemma:error-in-R-when-usin-representative-states} and \ref{lemma:error-in-bonus-when-usin-representative-states}. 
%	
%	By the construction of \RSkerns, we have
%	\begin{align*}
%		\max_{s'\in[k-1]} \dist{(x_h^{s'},a_h^{s'}),\maptoReprSA(x_h^{s'},a_h^{s'})} \leq \maxdist
%		,\quad 
%		\max_{s'\in[k-1]}\Sdist{x_{h+1}^{s'}, \maptoReprS(x_{h+1}^{s'})} \leq \Smaxdist.
%	\end{align*}
%	Consequently,
%	\begin{align*}
%	& \tQ_{h}^k(x_h^s, a_h^s) -\tQ_{h, \mapzeta}^k(x_h^s, a_h^s) \lesssim  \epsilon_{h+1} +  \lipQ\Smaxdist +  \frac{\maxdist}{\ksigma}H.
%	\end{align*}
%	Now, take an arbitrary $(x, a)$. By Lemma \ref{lemma:technical-inequality-for-KeRNS-with-minimum},
%	\begin{align*}
%		\algQ_{h, \mapzeta}^k(x, a) & = \underset{(\bx,\ba) \in\ReprStates\times\ReprActions }{\min}\pa{\tQ_{h, \mapzeta}^k(\bx,\ba)+\lipQ \dist{(x,a), (\bx,\ba)}} \\
%		& = \underset{s\in[k-1], h\in[H]}{\min}\pa{\tQ_{h, \mapzeta}^k(x_h^s, a_h^s)+\lipQ \dist{(x,a), \maptoReprSA(x_h^s, a_h^s)}} 
%	\end{align*}
%	and, by definition,
%	\begin{align*}
%		\algQ_{h}^k(x, a)= \underset{s\in[k-1], h\in[H]}{\min}\pa{\tQ_{h}^k(x_h^s, a_h^s)+\lipQ \dist{(x,a), (x_h^s, a_h^s)}},
%	\end{align*}
%	we obtain, for any $(x, a)$,
%	\begin{align*}
%		& \abs{\algQ_{h}^k(x, a) - \algQ_{h, \mapzeta}^k(x, a)} \\
%		&  \lesssim 
%	    \min_{s\in[k-1], h\in[H]}\abs{ \tQ_{h}^k(x_h^s, a_h^s) -  \tQ_{h, \mapzeta}^k(x_h^s, a_h^s) } 
%		 + \lipQ \min_{s\in[k-1], h\in[H]}\abs{ \dist{(x,a), (x_h^s, a_h^s)} - \dist{(x,a), \maptoReprSA(x_h^s, a_h^s)}} \\
%		& \leq \epsilon_{h+1} +  \lipQ\Smaxdist +  \frac{\maxdist}{\ksigma}H + \lipQ \max_{s\in[k-1]}\dist{ (x_h^s, a_h^s), \maptoReprSA(x_h^s, a_h^s) } \\
%		& \leq \epsilon_{h+1} +  \lipQ(\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H = \epsilon_h.
%	\end{align*}
%	
%	which concludes the proof.
%\end{proof}

%\begin{ftheorem}[UCRL-type regret bound for \RSkerns]
%	\label{theorem:regret-RS-kerns-ucrl-type}
%	With probability at least $1-\cdelta$, the regret of \RSkerns is bounded as follows
%	\begin{align*}
%		\regret^{\RSkerns}(K) \lesssim   \regret_1^{\kerns}(K) + \lipQ(\maxdist + \Smaxdist)KH^2 + \frac{\maxdist}{\ksigma}KH^3.
%	\end{align*}
%	where $\regret_1^{\kerns}(K)$ is the UCRL-type regret bound given in Theorem \ref{theorem:regret-bound-ucrl-type} for \kerns.
%\end{ftheorem}
%\begin{proof} 
%	Let $\pi_k^{\mapzeta}$ be the policy followed by \RSkerns in episode $k$ and let  $\delta_{h,\mapzeta}^k \eqdef \algV_{h, \mapzeta}^k(x_h^k) - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_h^k) $
%	
%	
%	\paragraph{Regret decomposition} Consider the following decomposition, also used in the proof of Lemma \ref{lemma:regret-in-terms-of-sum-of-bonus-ucrl-type}:
%	\begin{align*}
%	\delta_{h,\mapzeta}^k 
%		& =  \algV_{h,\mapzeta}^k(x_h^k) - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_h^k) \\
%		%
%		& \leq \algQ_{h,\mapzeta}^k(x_h^k, a_h^k) - \trueQ_{k,h}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k) \\
%		%
%		& \leq \algQ_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueQ_{k,h}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k)
%		+ \lipQ\dist{(\tx_h^k, \ta_h^k), (x_h^k, a_h^k)}
%		,\quad\text{since $\algQ_{h,\mapzeta}^k$ is $\lipQ$-\lipschitz} \\
%		%
%		& \leq  \tQ_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueQ_{k,h}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k)
%		+ \lipQ\dist{(\tx_h^k, \ta_h^k), (x_h^k, a_h^k)}
%		,\quad\text{since $\algQ_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) \leq  \tQ_{h,\mapzeta}^k(\tx_h^k, \ta_h^k)$} \\
%		%
%		& = \estR_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueR_h^k(x_h^k, a_h^k) 
%		+  \estP_{h,\mapzeta}^k\algV_{h+1}^k(\tx_h^k, \ta_h^k) - \trueP_h^k\trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k)
%		+\bonus_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) 
%		+ \lipQ\dist{(\tx_h^k, \ta_h^k), (x_h^k, a_h^k)} \\
%		%
%		& = \quad 
%		    \underbrace { 
%		    	\estR_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueR_h^k(x_h^k, a_h^k) 
%		    }_{\termA} 
%		  + 
%			\underbrace{
%			\sqrbrackets{\estP_{h,\mapzeta}^k -\trueP_h^k}\trueV_{k,h+1}^* (\tx_h^k, \ta_h^k)
%		}_{\termB}
%		 + 
%			\underbrace{
%		\sqrbrackets{\estP_{h,\mapzeta}^k -\trueP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) 
%			}_{\termC} \\
%		&  + \underbrace{ 
%			\trueP_h^k \algV_{h+1,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueP_h^k\trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k)
%				}_{\termD}
%	    +\bonus_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) 
%		+ 2\lipQ\dist{(\tx_h^k, \ta_h^k), (x_h^k, a_h^k)}.
%	\end{align*}
%	
%	We will use the following results, which are a consequence of Lemmas  \ref{lemma:error-in-P-when-usin-representative-states}, \ref{lemma:error-in-R-when-usin-representative-states} and \ref{lemma:error-in-bonus-when-usin-representative-states}:
%	\begin{align*}
%		\abs{\estR_h^k(\tx_h^k, \ta_h^k) - \estR_{h,\mapzeta}^k(\tx_h^k, \ta_h^k)} 
%		& \leq  \frac{4}{\ksigma}\pa{1+\sqrt{\logplus(k/\kbeta)}}\pa{ \dist{(\tx_h^k, \ta_h^k),\maptoReprSA(\tx_h^k, \ta_h^k)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)} } \\
%		& \leq \frac{8\maxdist}{\ksigma}\pa{1+\sqrt{\logplus(k/\kbeta)}}\lesssim \frac{\maxdist}{\ksigma}.
%	\end{align*}
%	\begin{align*}
%		\bonus_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) & = \bonus_h^k(\tx_h^k, \ta_h^k) + \bonus_{h,\mapzeta}^k(\tx_h^k, \ta_h^k)  - \bonus_h^k(\tx_h^k, \ta_h^k)  \\
%		& \lesssim \bonus_h^k(\tx_h^k, \ta_h^k) + \frac{H}{\ksigma}\pa{1+\frac{1}{2 \kbeta^{1/2}}}\pa{ \dist{(\tx_h^k, \ta_h^k),\maptoReprSA(\tx_h^k, \ta_h^k)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)}} \\
%		& \lesssim \bonus_h^k(\tx_h^k, \ta_h^k) +\frac{\maxdist}{\ksigma}H.
%	\end{align*}
%	and, for any function $f$ that is $\lipQ$-\lipschitz and bounded by $H$,
%	\begin{align*}
%		& \abs{\pa{\estP_h^k - \estP_{h,\mapzeta}^k}f(\tx_h^k, \ta_h^k)} 
%		 \\
%	    &  \lesssim \lipQ \max_{s\in[k-1]}\Sdist{x_{h+1}^s, \maptoReprS(x_{h+1}^s)} 
%		 + \frac{4H}{\ksigma}\pa{ \dist{(\tx_h^k, \ta_h^k),\maptoReprSA(\tx_h^k, \ta_h^k)} + \max_{s\in[k-1]} \dist{(x_h^s,a_h^s),\maptoReprSA(x_h^s,a_h^s)} }\\
%		& \lesssim \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H.
%	\end{align*}
%	
%	Now, we bound each term $\termA-\termD$.
%	
%	\underline{Term $\termA$}: by Lemma \ref{lemma:error-in-R-when-usin-representative-states}, the definition of $\goodevent$ and Corollary \ref{corollary:bias-between-avmdp-and-true-mdp}, we have
%	\begin{align*}
%		\termA & = \estR_{h,\mapzeta}^k(\tx_h^k, \ta_h^k) - \estR_h^k(\tx_h^k, \ta_h^k) + \estR_h^k(\tx_h^k, \ta_h^k) - \trueR_h^k(\tx_h^k, \ta_h^k) + \trueR_h^k(\tx_h^k, \ta_h^k) - \trueR_h^k(x_h^k, a_h^k) \\
%		& \lesssim \frac{\maxdist}{\ksigma} + \estR_h^k(\tx_h^k, \ta_h^k) - \trueR_h^k(\tx_h^k, \ta_h^k) + \trueR_h^k(\tx_h^k, \ta_h^k) - \trueR_h^k(x_h^k, a_h^k) \\
%		& \leq \frac{\maxdist}{\ksigma} +  \rbonus_h^k(\tx_h^k, \ta_h^k) + \biasR(k, h) +\lipR \dist{(\tx_h^k, \ta_h^k), (x_h^k, a_h^k)}.
%	\end{align*}
%	
%
%	\underline{Term $\termB$}:
%	\begin{align*}
%	\termB & = \sqrbrackets{\estP_{h,\mapzeta}^k -\estP_h^k}\trueV_{k,h+1}^* (\tx_h^k, \ta_h^k) + \sqrbrackets{\estP_h^k -\trueP_h^k}\trueV_{k,h+1}^* (\tx_h^k, \ta_h^k)\\ 
%	& \lesssim \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H + \sqrbrackets{\estP_h^k -\avP_h^k}\trueV_{k,h+1}^* (\tx_h^k, \ta_h^k) + 
%	\sqrbrackets{\avP_h^k -\trueP_h^k}\trueV_{k,h+1}^* (\tx_h^k, \ta_h^k) \\
%	& \leq \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H + \pbonus_h^k(\tx_h^k, \ta_h^k) + \biasP(k, h)
%	\end{align*}
%	
%
%	\underline{Term $\termC$}: Using Corollary \ref{corollary:bias-between-avmdp-and-true-mdp}, we obtain
%	\begin{align*}
%		\termC &= \sqrbrackets{\estP_{h,\mapzeta}^k -\trueP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) \\
%		&= \sqrbrackets{\estP_{h,\mapzeta}^k -\estP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) + \sqrbrackets{\estP_h^k -\trueP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k)  \\
%		& \lesssim  \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H +  \sqrbrackets{\estP_h^k -\avP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) + \biasP(k, h) \\
%		& \lesssim \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H +  \sqrt{  \frac{ H^2 \Xsigmacov }{\gencount_h^k(\tx_h^k, \ta_h^k)} }
%		+ \frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)}  + \lipQ \ksigma + \biasP(k, h)
%	\end{align*}
%	by the definition of $\goodevent$.
%	
%
%	\underline{Term $\termD$}: From Assumption \ref{assumption:lipschitz-rewards-and-transitions}, for any $\lipQ$-\lipschitz function, the mapping $(x, a) \mapsto \trueP_h^k f(x, a)$ is $\lipP\lipQ$-\lipschitz. Consequently,
%	\begin{align*}
%		\termD & =  \trueP_h^k \algV_{h+1,\mapzeta}^k(\tx_h^k, \ta_h^k) - \trueP_h^k\trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k)\\
%		& \leq \trueP_h^k \algV_{h+1,\mapzeta}^k(x_h^k, a_h^k) - \trueP_h^k\trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_h^k, a_h^k) + \lipP\lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)}\\
%		& = \trueP_h^k\pa{ \algV_{h+1,\mapzeta}^k - \trueV_{k,h+1}^{\pi_k^{\mapzeta}}}(x_h^k, a_h^k) + \lipP\lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \\
%		& = \delta_{h+1}^k + \xi_{h+1}^k + \lipP\lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)}.
%	\end{align*}
%	where 
%	\begin{align*}
%	\xi_{h+1}^k \eqdef  \trueP_h^k\pa{ \algV_{h+1,\mapzeta}^k - \trueV_{k,h+1}^{\pi_k^{\mapzeta}}}(x_h^k, a_h^k) - \delta_{h+1,\mapzeta}^k
%	\end{align*}
%	is a martingale difference sequence with respect to $(\cF_h^k)_{k, h}$ bounded by $4H$. 
%	
%	Putting together the bounds for $\termA$-$\termD$ and using the definition of the bonuses $\bonus_h^k$, we obtain
%	\begin{align*}
%		\delta_{h,\mapzeta}^k \lesssim
%		& \delta_{h+1,\mapzeta}^k + \xi_{h+1}^k 
%		+ \lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)}
%		+ \sqrt{  \frac{ H^2 \Xsigmacov }{\gencount_h^k(\tx_h^k, \ta_h^k)} } \\
%		& + \frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)} 
%		+ \lipQ\ksigma  
%		+ \bias(k, h')
%		+ \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H
%	\end{align*}
%		where the constant in front of $\delta_{h+1,\mapzeta}^k$ is \emph{exact} (\ie not omitted by $\lesssim$). 
%		
%	Now, we follow the same arguments as in the proof of Lemma \ref{lemma:regret-in-terms-of-sum-of-bonus-ucrl-type}. Consider the event $E_h^k \eqdef \braces{\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \leq  2 \ksigma}$. The inequality above gives us
%	\begin{align}
%        \indic{E_h^k}\delta_{h,\mapzeta}^k \lesssim
%		&  \indic{E_h^k} \delta_{h+1,\mapzeta}^k +  \indic{E_h^k}\xi_{h+1}^k 
%		+  \indic{E_h^k}\sqrt{  \frac{ H^2 \Xsigmacov }{\gencount_h^k(\tx_h^k, \ta_h^k)} } \nonumber \\
%		& +  \indic{E_h^k}\frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)} 
%		+ 3\lipQ\ksigma  
%		+ \bias(k, h')
%		+ \lipQ\Smaxdist +\frac{\maxdist}{\ksigma}H 		\label{eq:rs-kerns-delta-trick}.
%	\end{align}
%	
%	Using Lemmas \ref{lemma:upper-bound-on-q-functions} and \ref{lemma:diff-between-Q-in-kerns-and-RS-kerns}, we upper bound $ \indic{E_h^k} \delta_{h+1,\mapzeta}^k$ in terms of $\delta_{h+1,\mapzeta}^k$:
%	\begin{align}
%		\indic{E_h^k} \delta_{h+1,\mapzeta}^k
%		&
%		 = \indic{E_h^k}\pa{ \algV_{h+1,\mapzeta}^k(x_{h+1}^k) - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_{h+1}^k)} 
%		 \nonumber
%		\\
%		&
%		\lesssim \indic{E_h^k}\pa{ 
%			H\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H^2
%			+ \algV_{h+1}^k(x_{h+1}^k) - \trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_{h+1}^k)
%		} 
%		\nonumber
%		\\
%		& 
%		\leq H\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H^2
%		+ \indic{E_h^k}
%		\underbrace{
%		\pa{ 
%			  \algV_{h+1}^k(x_{h+1}^k) + \sum_{h'=h+1}^H \bias(k, h)  - \trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_{h+1}^k)
%		} 
%	}_{\geq 0 \text{ by Lemma \ref{lemma:upper-bound-on-q-functions}}}
%		\nonumber
%       \\
%       & 
%       \leq 
%        H\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H^2
%        + \algV_{h+1}^k(x_{h+1}^k) -  \trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_{h+1}^k)
%        + \sum_{h'=h+1}^H \bias(k, h)
%        \nonumber
%       \\
%       & 
%       \leq 
%       2H\lipQ (\maxdist + \Smaxdist) + 2\frac{\maxdist}{\ksigma}H^2
%       + \algV_{h+1,\mapzeta}^k(x_{h+1}^k) -  \trueV_{k,h+1}^{\pi_k^{\mapzeta}}(x_{h+1}^k)
%       + \sum_{h'=h+1}^H \bias(k, h) 
%       \nonumber
%       \\
%		&
%	   = \delta_{h+1,\mapzeta}^k        
%	   + 2H\lipQ (\maxdist + \Smaxdist) + 2\frac{\maxdist}{\ksigma}H^2
%	   + \sum_{h'=h+1}^H \bias(k, h)
%	   \label{eq:rs-kerns-delta-trick-two}
%	\end{align}
%	
%	Let $\overline{E}_h^k$ be the complement of $E_h^k$. Using the inequality above combined with \eqref{eq:rs-kerns-delta-trick}, and the fact that $\delta_{h,\mapzeta}^k \leq H$, we obtain
%	\begin{align}
%	\delta_{h,\mapzeta}^k 
%	& = \indic{\overline{E}_h^k}\delta_{h,\mapzeta}^k  + \indic{E_h^k}\delta_{h,\mapzeta}^k 
%	\label{eq:rs-kerns-delta-trick-three}
%	\\
%	& 
%	\leq  H \indic{\overline{E}_h^k} + \indic{E_h^k}\delta_{h,\mapzeta}^k 
%	\nonumber
%	\\
%	& 
%	\lesssim  
%	 H \indic{\overline{E}_h^k}
%	 + \delta_{h+1,\mapzeta}^k        
%	 + H\lipQ (\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}H^2
%	 + \sum_{h'=h}^H \bias(k, h)
%	 +  \indic{E_h^k}\xi_{h+1}^k
%	 \nonumber 
%	 \\
%	 & 
%	+  \indic{E_h^k}\sqrt{  \frac{ H^2 \Xsigmacov }{\gencount_h^k(\tx_h^k, \ta_h^k)} } 
%	 +  \indic{E_h^k}\frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)} 
%	 + \lipQ\ksigma  
%	 \nonumber
%	\end{align}
%	
%	
%	Consequently, 
%	\begin{align*}
%		\sum_{k=1}^K \delta_{1,\mapzeta}^k \lesssim & 
%		\sum_{k=1}^K\sum_{h=1}^H \pa{\frac{H\sqrt{\Xsigmacov}}{\sqrt{\gencount_h^k(\tx_h^k, \ta_h^k)}} 
%			+  \frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)} }\indic{E_h^k}
%		+ H \sum_{k=1}^K\sum_{h=1}^H \indic{\overline{E}_h^k}  \\
%		& +  \sum_{k=1}^K\sum_{h=1}^H \indic{E_h^k} \xi_{h+1}^k 
%		+  H \sum_{k=1}^K\sum_{h=1}^H \bias(k, h) 
%		+ \lipQ (\maxdist + \Smaxdist)KH^2 + \frac{\maxdist}{\ksigma}KH^3
%	\end{align*}
%
%	
%	Now, as in the proof of Lemma  \ref{lemma:regret-in-terms-of-sum-of-bonus-ucrl-type}, we show that 
%	\begin{align*}
%		 H \sum_{k=1}^K\sum_{h=1}^H \indic{\overline{E}_h^k} \leq H^2\sigmacov
%	\end{align*}
%	
%	and, from lemmas \ref{lemma:upper-bound-on-q-functions} and \ref{lemma:diff-between-Q-in-kerns-and-RS-kerns}, we have:
%	\begin{align*}
%	\regret^{\RSkerns}(K) & = \sum_{k=1}^{K} \pa{\trueV_{k,1}^*(x_1^k) - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} \\
%	& \leq \sum_{k=1}^{K}\pa{ \algV_{1}^k(x_1^k)  - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) \\
%	& \lesssim  \sum_{k=1}^{K}\pa{ \algV_{1,\mapzeta}^k(x_1^k)  - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) + \lipQ KH(\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}KH^2 \\
%	& =  \sum_{k=1}^K \delta_{1,\mapzeta}^k + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) + \lipQ KH(\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}KH^2 \\
%	& \lesssim \sum_{k=1}^K\sum_{h=1}^H \pa{\frac{H\sqrt{\Xsigmacov}}{\sqrt{\gencount_h^k(\tx_h^k, \ta_h^k)}} 
%		+  \frac{\kbeta H}{\gencount_h^k(\tx_h^k, \ta_h^k)} }\indic{E_h^k}
%	+ H^2\sigmacov  \\
%	& +  \sum_{k=1}^K\sum_{h=1}^H \indic{E_h^k} \xi_{h+1}^k 
%	+  H \sum_{k=1}^K\sum_{h=1}^H \bias(k, h) 
%	+ \lipQ (\maxdist + \Smaxdist)KH^2 + \frac{\maxdist}{\ksigma}KH^3.
%	\end{align*}
%
%	Recall the definition $E_h^k \eqdef \braces{\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \leq  2 \ksigma}$ and the fact that $\widetilde{\xi}_{h+1}^k\eqdef \indic{E_h^k} \xi_{h+1}^k$ is a martingale difference sequence with respect to $(\cF_h^k)_{k, h}$ bounded by $4H$. 
%	Then, as in the proof of Theorem \ref{theorem:regret-bound-ucrl-type}, we obtain
%	
%	\begin{align*}
%		\regret^{\RSkerns}(K) \lesssim & \regret_1^{\kerns}(K) +  \lipQ KH^2 (\maxdist + \Smaxdist) +\frac{\maxdist}{\ksigma} KH^3
%	\end{align*}
%	with probability at least $1-\cdelta$.
%\end{proof}


%\begin{ftheorem}[UCBVI-type regret bound for \RSkerns]
%	\label{theorem:regret-RS-kerns-ucbvi-type}
%	With probability at least $1-\cdelta$, the regret of \RSkerns is bounded as follows
%	\begin{align*}
%	\regret^{\RSkerns}(K) \lesssim   \regret_2^{\kerns}(K) + \lipQ(\maxdist + \Smaxdist)KH^2 + \frac{\maxdist}{\ksigma}KH^3.
%	\end{align*}
%	where $\regret_2^{\kerns}(K)$ is the UCBVI-type regret bound given in Theorem \ref{theorem:regret-bound-ucbvi-type} for \kerns.
%\end{ftheorem}
%
%\begin{proof}
%	We use the same regret decomposition as in the proof of Theorem \ref{theorem:regret-RS-kerns-ucrl-type}, but the term $\termC$ is bounded differently (as in Lemma \ref{lemma:regret-in-terms-of-sum-of-bonus}).
%	
%	Using Lemma \ref{lemma:diff-between-Q-in-kerns-and-RS-kerns} and the same arguments as in the proof of Lemma \ref{lemma:regret-in-terms-of-sum-of-bonus}, we have
%	\begin{align*}
%	\termC 
%	& = \sqrbrackets{\estP_h^k -\trueP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) \\
%	%
%	& = \sqrbrackets{\estP_h^k -\trueP_h^k}\pa{ \algV_{h+1,\mapzeta}^k- \algV_{h+1}^k}(\tx_h^k, \ta_h^k) 
%	+ \sqrbrackets{\estP_h^k -\trueP_h^k}\pa{ \algV_{h+1}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) \\
%	%
%	& \leq 2 \lipQ (\maxdist + \Smaxdist)H + 2\frac{\maxdist}{\ksigma}H^2 + \sqrbrackets{\estP_h^k -\trueP_h^k}\pa{ \algV_{h+1}^k- \trueV_{k,h+1}^*}(\tx_h^k, \ta_h^k) \\
%	%
%	& \lesssim   \lipQ (\maxdist + \Smaxdist)H + \frac{\maxdist}{\ksigma}H^2 +  \frac{1}{H} \trueP_h^k\pa{ \algV_{h+1}^k- \trueV_{k,h+1}^*}(x_h^k, a_h^k) + \frac{H^2\Xsigmacov}{\gencount_h^k(\tx_h^k, \ta_h^k)} \\
%	   & + \lipQ\ksigma +  \sum_{h'=h}^H \bias(k, h') + \lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \\
%	%
%	& \lesssim   \lipQ (\maxdist + \Smaxdist)H + \frac{\maxdist}{\ksigma}H^2 +  \frac{1}{H} \trueP_h^k\pa{ \algV_{h+1}^k- \trueV_{k,h+1}^{\pi_k^{\mapzeta}}}(x_h^k, a_h^k) + \frac{H^2\Xsigmacov}{\gencount_h^k(\tx_h^k, \ta_h^k)} \\
%	& + \lipQ\ksigma +  \sum_{h'=h}^H \bias(k, h') + \lipQ\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)}
%	\end{align*}
%	where, in the last line, we used the fact that $\trueV_{k,h+1}^{\pi_k^{\mapzeta}} \leq \trueV_{k,h+1}^*$.
%
%	Putting together the bounds for $\termA-\termD$ and using the same arguments as in the proof of Theorem \ref{theorem:regret-RS-kerns-ucrl-type}, especially the inequalities \eqref{eq:rs-kerns-delta-trick}, \eqref{eq:rs-kerns-delta-trick-two} and \eqref{eq:rs-kerns-delta-trick-three}, we obtain
%
%	\begin{align*}
%		\sum_{k=1}^K \delta_{1,\mapzeta}^k \lesssim & 
%		\sum_{k=1}^K\sum_{h=1}^H \pa{\frac{H}{\sqrt{\gencount_h^k(\tx_h^k, \ta_h^k)}} 
%			+  \frac{H^2\Xsigmacov}{\gencount_h^k(\tx_h^k, \ta_h^k)} }\indic{\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \leq  2 \ksigma}
%		+ H^2 \sigmacov \\
%		& +  \sum_{k=1}^K\sum_{h=1}^H \pa{1+\frac{1}{H}}^{H-h+1}\widetilde{\xi}_{h+1}^k 
%		+  H \sum_{k=1}^K\sum_{h=1}^H \bias(k, h) 
%		+ \lipQ K H\ksigma 
%		+ \lipQ (\maxdist + \Smaxdist)H^2 + \frac{\maxdist}{\ksigma}H^3
%	\end{align*}
%
%	where $\widetilde{\xi}_{h+1}^k$	is a martingale difference sequence with respect to $(\cF_h^k)_{k, h}$ bounded by $4H$. 
%
%
%
%	Now, from lemmas \ref{lemma:upper-bound-on-q-functions} and \ref{lemma:diff-between-Q-in-kerns-and-RS-kerns} , we have:
%	\begin{align*}
%		\regret^{\RSkerns}(K) & = \sum_{k=1}^{K} \pa{\trueV_{k,1}^*(x_1^k) - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} 
%		 \leq \sum_{k=1}^{K}\pa{ \algV_{1}^k(x_1^k)  - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) \\
%		& \lesssim  \sum_{k=1}^{K}\pa{ \algV_{1,\mapzeta}^k(x_1^k)  - \trueV_{k,h}^{\pi_k^{\mapzeta}}(x_1^k)} + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) + \lipQ KH(\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}KH^2 \\
%		& =  \sum_{k=1}^K \delta_{1,\mapzeta}^k + \sum_{k=1}^{K}\sum_{h=1}^H \bias(k, h) + \lipQ KH(\maxdist + \Smaxdist) + \frac{\maxdist}{\ksigma}KH^2 \\
%		& \lesssim 		\sum_{k=1}^K\sum_{h=1}^H \pa{\frac{H}{\sqrt{\gencount_h^k(\tx_h^k, \ta_h^k)}} 
%			+  \frac{H^2\Xsigmacov}{\gencount_h^k(\tx_h^k, \ta_h^k)} }\indic{\dist{(x_h^k, a_h^k), (\tx_h^k, \ta_h^k)} \leq  2 \ksigma}
%		+ H^2 \sigmacov \\
%		& +  \sum_{k=1}^K\sum_{h=1}^H \pa{1+\frac{1}{H}}^{h}\widetilde{\xi}_{h+1}^k 
%		+  H \sum_{k=1}^K\sum_{h=1}^H \bias(k, h) 
%		+ \lipQ K H\ksigma 
%		+ \lipQ (\maxdist + \Smaxdist)KH^2 + \frac{\maxdist}{\ksigma}KH^3
%	\end{align*}
%	
%	Then, as in the proof of Theorem \ref{theorem:regret-bound-ucbvi-type}, we obtain
%	
%	\begin{align*}
%	\regret^{\RSkerns}(K) \lesssim & \regret_2^{\kerns}(K) +  \lipQ (\maxdist + \Smaxdist)KH^2  +\frac{\maxdist}{\ksigma} KH^3
%	\end{align*}
%	with probability at least $1-\cdelta$.
%\end{proof}



